PolSAM: Polarimetric Scattering Mechanism Informed Segment Anything Model

PolSAR data presents unique challenges due to its rich and complex characteristics. Existing data representations, such as complex-valued data, polarimetric features, and amplitude images, are widely used. However, these formats often face issues related to usability, interpretability, and data integrity. Most feature extraction networks for PolSAR are small, limiting their ability to capture features effectively. To address these issues, We propose the Polarimetric Scattering Mechanism-Informed SAM (PolSAM), an enhanced Segment Anything Model (SAM) that integrates domain-specific scattering characteristics and a novel prompt generation strategy. PolSAM introduces Microwave Vision Data (MVD), a lightweight and interpretable data representation derived from polarimetric decomposition and semantic correlations. We propose two key components: the Feature-Level Fusion Prompt (FFP), which fuses visual tokens from pseudo-colored SAR images and MVD to address modality incompatibility in the frozen SAM encoder, and the Semantic-Level Fusion Prompt (SFP), which refines sparse and dense segmentation prompts using semantic information. Experimental results on the PhySAR-Seg datasets demonstrate that PolSAM significantly outperforms existing SAM-based and multimodal fusion models, improving segmentation accuracy, reducing data storage, and accelerating inference time. The source code and datasets will be made publicly available at https://github.com/XAI4SAR/PolSAM.

==> bios.tex <==
Author Biographies and Photo Mapping — TCSVT-27254-2025

1. Yuqing Wang — Figures/wang.jpg
Yuqing Wang is currently working toward the Ph.D. degree in the School of Automation, Northwestern Polytechnical University, Xi'an, China. Her research interests include computer vision, synthetic aperture radar (SAR) image interpretation, multimodal image fusion, medical image processing, and adaptation of foundation models.

2. Zhongling Huang — Figures/huang.png
Zhongling Huang (huangzhongling@nwpu.edu.cn) received her B.Sc. degree in electronic information science and technology from Beijing Normal University, Beijing, China, in 2015, and her Ph.D. degree from the University of Chinese Academy of Sciences (UCAS) and the Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing, China, in 2020. She served as a visiting scholar in the German Aerospace Center during 2018–2019, funded by UCAS. She is currently working in the Brain and Artificial Intelligence Lab, School of Automation, Northwestern Polytechnical University, Xi’an 710072, China. Her research interests include explainable deep learning for synthetic aperture radar (SAR), SAR image interpretation, deep learning, and remote sensing data mining.

3. Shuxin Yang — Figures/yang.jpg
Shuxin Yang is currently a master's student at Northwestern Polytechnical University in Xi'an, Shanxi. His research direction is SAR image target detection in computer vision.

4. Hao Tang — Figures/tang.png
is an Assistant Professor at Peking University, China. Previously, he held postdoctoral positions at both CMU, USA, and ETH Zürich, Switzerland. He earned a master's degree from Peking University, China, and a Ph.D. from the University of Trento, Italy. He was a visiting Ph.D. student at the University of Oxford, UK, and an intern at IIAI, UAE. His research interests include machine learning, computer vision, embodied AI, and AIGC (including LLM), as well as their applications in scientific domains.

5. Xiaolan Qiu (Senior Member, IEEE) — Figures/qiu.png
Xiaolan Qiu (Senior Member, IEEE) received the B.S. degree in electronic engineering and information science from the University of Science and Technology of China, Hefei, China, in 2004, and the Ph.D. degree in signal and information processing from the Graduate University of Chinese Academy of Sciences, Beijing, China, in 2009. She is with the National Key Laboratory of Microwave Imaging Technology, Chinese Academy of Sciences, Beijing 100090, China, and also with the Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing 100094, China. Her research interests include synthetic aperture radar (SAR) imaging, SAR simulation, and SAR 3-D reconstruction.

6. Junwei Han (Fellow, IEEE) — Figures/han.png
Junwei Han (Fellow, IEEE) is currently a Professor in the School of Automation, Northwestern Polytechnical University. His research interests include computer vision, pattern recognition, remote sensing image analysis, and brain imaging analysis. He has published more than 70 papers in top journals such as IEEE TPAMI, TNNLS, IJCV, and more than 30 papers in top conferences such as CVPR, ICCV, MICCAI, and IJCAI. He is an Associate Editor for several journals such as IEEE TNNLS and IEEE TMM.

7. Dingwen Zhang (Member, IEEE) — Figures/zhang.png
Dingwen Zhang (Member, IEEE) received the Ph.D. degree from Northwestern Polytechnical University, Xi’an, China, in 2018. He is a Professor with the School of Automation, Northwestern Polytechnical University. From 2015 to 2017, he was a Visiting Scholar with the Robotic Institute, Carnegie Mellon University, Pittsburgh, PA, USA. His research interests include computer vision and multimedia processing, especially on saliency detection and weakly supervised learning.



